FLAME: Federated Learning Across Multi-device Environments

Federated Learning (FL) enables distributed training of machine learning models while keeping personal data on user devices private. While we witness increasing applications of FL in the area of mobile sensing, such as human activity recognition (HAR), FL has not been studied in the context of a multi-device environment (MDE), wherein each user owns multiple data-producing devices. With the proliferation of mobile and wearable devices, MDEs are increasingly becoming popular in ubicomp settings, therefore necessitating the study of FL in them. FL in MDEs is characterized by being not independent and identically distributed (non-IID) across clients, complicated by the presence of both user and device heterogeneities. Further, ensuring efficient utilization of system resources on FL clients in a MDE remains an important challenge. In this paper, we propose FLAME, a user-centered FL training approach to counter statistical and system heterogeneity in MDEs, and bring consistency in inference performance across devices. FLAME features (i) user-centered FL training utilizing the time alignment across devices from the same user; (ii) accuracy- and efficiency-aware device selection; and (iii) model personalization to devices. We also present an FL evaluation testbed with realistic energy drain and network bandwidth profiles, and a novel class-based data partitioning scheme to extend existing HAR datasets to a federated setup. Our experiment results on three multi-device HAR datasets show that FLAME outperforms various baselines by 4.3-25.8% higher F1 score, 1.02-2.86x greater energy efficiency, and up to 2.06x speedup in convergence to target accuracy through fair distribution of the FL workload.

==> 10_revision_summary.tex <==
\newpage
\clearpage
\setcounter{section}{0}
% \renewcommand\thesection{1AE.\arabic{section}}
\vspace{-0.2cm}
{\noindent \huge \textbf{List of Revisions}}

\vspace{0.2cm}
{\noindent We thank the reviewers for the detailed reviews and constructive suggestions to improve our paper. We summarize the changes we made in this revision and how we addressed the comments from each reviewer. In addition to the changes summarized below, we further proofread and revised the draft. The comments from 2AE~(R1), R3, R4, and R5 that were echoed by 1AE~(R2) and revisions for those comments are summarized and annotated with the name of related reviewers in the subsection titles.}

\section{Presentation [R3, R4]}
\begin{enumerate}[label=(\alph*)]
    \item We have increased the readability of Figure 4 by increasing the line thickness, font sizes, and enlarging the graphics. 
    \item We added two sentences to explain Figure 4 at the end of \S3.2.
    \item We added a reference for MDE (Multi-Device Environment) from \S4.1 to the definition in \S\ref{sec:problem}. The header for defining MDE was also shortened from ``Definition 3.1 (Multi-device Environment (MDE))'' to ``Multi-Device Environment (MDE)'' for better visibility.     
    \item In \S\ref{sec:client_selection}, we added 1-2 sentences to the end of each utility's paragraph to clarify the ranges and indication whether a higher/lower utility is good/bad. We also added Table~\ref{tab:utility_info} in Appendix.
    \item We added the definition of a \dead{} device in the bullet point list of \S\ref{sec:evaluation} as well as reference to \S\ref{sec:eval_metrics} for details.
\end{enumerate}

\section{Motivation [R5]}
\textit{``R5 is not convinced about the current motivation of the paper and suggests a different motivation. Please, strengthen your motivation''}

\parjump{}
\noindent
\textbf{Response:} Our work is motivated by the emerging ecosystem of multi-device environments, where a user owns multiple data generating devices, e.g., a smartphone, a smart watch, a smart ring, a smart earbud. Our underlying assumption is that these devices do not share their raw sensor data with other devices due to privacy, proprietary, or legal reasons. As such, we need a (federated) learning approach which can train ML models on the data distributed on these devices, while respecting the privacy of each device's data. 

\parjump{}
\noindent
In the current market landscape, there are a number of such devices that support this assumption. For example, Oura Ring\footnote{https://ouraring.com/} is a popular wearable device that does activity, health, and sleep tracking, but does not allow users to access raw sensor data. Similarly, Apple Airpods and Amazon Echo Frames smart glasses contain a number of important sensors such as accelerometers, gyroscopes that can be used for HAR; however, the devices do not allow access to raw sensor data. We envision that the line of research proposed in our paper could allow such devices to collaborate with each other (and with other users) to train robust HAR models, while ensuring that the raw data stay on the device.      

\parjump{}
\noindent
At the same time, we do not discount the viewpoint put forth by R5 and also hinted by R1 (2AE). It is possible that future regulations may compel device manufacturers to give the users access to their raw sensor data. In such cases, the sensor data from each device can be streamed and stored at a common device (e.g., smartphone) in an energy-efficient manner, and HAR models can be trained locally on the smartphone or in a federated manner using single-device FL approaches. 

\parjump{}
\noindent
We believe both of the above are plausible ways in which multi-device ecosystems can evolve, and as researchers, we should investigate both of them. This paper focuses on the first scenario, and we leave the other scenario for future work. We have summarized this reasoning in \S\ref{sec:introduction} to strengthen our motivation. Fortuitously, we are also seeing improvements in ML training support for resource-constrained devices, e.g., using TensorFlow Lite's optimized on-device training\footnote{\url{https://www.tensorflow.org/lite/examples/on_device_training/overview}}. Such software enhancements should enable more explorations of local or federated training on mobile and wearable devices.

\parjump{}
\noindent
Moreover, as R5 rightly points out, our investigation focuses on the uni-modal case, when all devices have inertial sensors. The exploration of multi-modal FL wherein devices may have different modalities of data is outside the scope of this work. We have added it as a limitation and opportunity for future work in \S\ref{sec:limitations}.

\section{Methodology [R3, R4, R5]}
%% R3
\subsection{Relationship of the SWD metric with FL accuracy [R3]}

Thanks for this question. We extended the experiment from Figure~\ref{fig:swd} and trained FL models in each of these settings to evaluate the impact of non-IID-ness on model accuracy. Our methodology was as follows: we chose test sets from the single-devices in our setup (`head' and `wrist') and evaluated the performance of single-device FL models on them. Recall that in this scenario there is no device heterogeneity, hence we expect higher model accuracy. Next, we took the model trained in a multi-device setup (with both user and device heterogeneity) and tested it on both the `head' and `wrist' test sets. 

Our results show that the FL model trained in the multi-device setting has an accuracy of 54.2\% and 52.6\% on the test sets of head and wrist respectively. In comparison, a model trained in the single-device setups of head and wrist obtain accuracies of 72.4\% and 67.3\% respectively on their test datasets. This finding confirms that the presence of both user and device heterogeneities in the multi-device setup lead to degradation in the performance of FL algorithms (by 18.2\% and 14.7\% respectively). We note that this accuracy drop follows the trend of increase in non-IID-ness, but is not directly proportional to it. 

\subsection{More details on enforcing time alignment [R3]}
R3: \textit{In Section 4.1, I wondered about the following sentence: ``It is observed that during the FL, if we enforce..., we can achieve faster convergence and higher overall accuracy.'' How realistic such enforcement in a real-world system? Are there any disadvantages of such approach, e.g., what happens if the data from one of devices is missing/incomplete?}

In practice, time alignment can be achieved through exchanging wall-clock time among co-located devices whose proximity could be known through various ways, e.g., bluetooth signal proximity. In more extreme scenarios where the data from one or more devices are missing or incomplete, previously collected data could be used instead; in the worst case, \system{} would perform as running with randomly shuffled data shown in Figure~\ref{fig:time_alignment_compare}.
We appended this explanation at the end of \S\ref{sec:user_centered_fl}.


\subsection{Measurement methods of execution time and energy consumptions [R3]}
Python's time module and Monsoon power monitor were used to measure the training time and energy level, respectively.

%% R4
\subsection{Energy consumption calculation not considering overconsumption [R4]}
As we define in \S\ref{sec:evaluation}, \system{} considers a device as `\dead{}' when its energy drain grows above a predefined drain threshold. \Dead{} devices are excluded from participating in federated training to prevent overconsumption. Therefore, the energy consumption of FL in our context is the sum of energy consumed on each of the client devices during training.

\subsection{Users owning different number of devices [R4]}
Our client selection algorithm takes into account cases where different users own different numbers of devices by selecting $max$($\rho$, number of available devices) per user. This also happened in our experiments since more devices go invalid as the training progresses. We continue sampling devices from more users until we sample $C$ devices in total in each round. Thanks to the comment, we added more accurate description of this process in \S\ref{sec:user_centered_fl} and \S\ref{sec:client_selection}.

\subsection{How metrics are computed before a device has been sampled [R4]}
We run the initial round with all participating devices. 


\section{Evaluation [R3, R5]}
%% R3

\subsection{Lower-end platforms and smartphones [R3]}
We primarily focused our experiments on Python-enabled devices due to their native support for ML \emph{training} frameworks. We also added some devices in our testbed, such as Jetson Nano and Raspberry Pi, which have significantly less run-time memory than modern smartphones. 

Based on the reviewer's suggestion, we have also evaluated the run-time performance of \system{} on Google Pixel 5 devices, by porting the model from Python to TensorFlow Lite and utilizing the newly released on-device training capabilities of TensorFlow Lite on Android. The results have been added to the Appendix and are also shown below: 
\begin{table}[h]
\small
\caption{Training time and energy consumption per round for training an HAR model on the partitioned RealWorld dataset on Google Pixel 5 Android device. We follow the same methodology as with other devices listed in Table~\ref{tab:energy_profiles}.}
\vspace{-0.3cm}
\label{tab:android}
\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{Name}                                                      & \textbf{Processor Type} & \textbf{Release Year} & \textbf{\begin{tabular}[c]{@{}c@{}}Training \\ time per round \\ (in seconds)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Energy consumption\\ per round \\ (in Joules)\end{tabular}} \\ \midrule
Google Pixel 5 & CPU & 2020 & 24.42 & 48.36\\  \bottomrule
\end{tabular}
\end{table}

We did not evaluate \system{} on Arduino as it currently does not have software support for ML training using Tensorflow or PyTorch. As a next step, we have started working on porting \system{} to C++, which will enable it to be deployed on a wider set of non-Python devices. 


\subsection{Justification of baseline selection [R3]}
We use FedAvg as a baseline as it is the original algorithm proposed for federated learning. Ditto is a state-of-the-art personalization extension of FedAvg that includes the training of personalized models. 
The initial experiment with FedAvg and Ditto and ablation study showed that personalization is a large contributor to higher macro-F1 score.
Therefore, we continued comparison with client selection baselines by substituting only the client selection strategy while preserving other parts of \system{} including personalization. 
We used Oort as a client selection baseline for being the state-of-the-art device selection policy that considers both statistical and time utility. 
In this revision, we also added \textsc{Power-of-choice} ($\pi_{pow-d}$) and its computation-efficient variant ($\pi_{cpow-d}$) to compare \system{} to another device selection strategy focusing on statistical utility ($\pi_{pow-d}$) and both statistical and computational utility ($\pi_{cpow-d}$).
We added these justifications to \S\ref{sec:baselines} as well.

\subsection{Representative number for device model speedups [R3]}
We added the representative numbers for the speedups for the device model in \S\ref{sec:results} as the following: ``Our results show that \system{} achieves speedups for the device models as they converge faster due to personalization with 2.06$\times$, 1.80$\times$, and 1.58$\times$ speedups, respectively for RealWorld, Opportunity, and PAMAP2 datasets.''

\subsection{Description of Oort [R3]}
We added more explanation in \S\ref{sec:analysis_flame} on how Oort defines its time utility as $(\frac{T}{t_i})^{\mathbbm{1}(T<t_i)\times\alpha}$ which favors clients with shorter training time $t_i$ when $t_i$ is greater than the preferred threshold $T$.

\subsection{Time alignment in ablation [R3]}
We originally included the effect of time alignment to show the importance of enforcing the time alignment. However, as R3 pointed out, this is a setup assumption in MDEs. Thus, we removed the `FLAME w/o Time Alignment' line from Figure \ref{fig:rw_ablation} and separated out to Figure \ref{fig:time_alignment_compare} in \S\ref{sec:user_centered_fl}.

\subsection{Criteria for selecting different datasets for evaluations [R3]}
In order to maintain the consistency of presenting the results as suggested by R3, we replaced the results for Figure \ref{fig:device_count} with the results using the RealWorld dataset.


%% R5
\subsection{Local finetuning as personalization for baseline [R5]}
R5 suggested adding local finetuning, where ``the clients leave their last energy portions to a local fine-tuning round.'' Following the suggestion, we added the results of applying local finetuning to FedAvg and \system{} models in the Appendix. Figure~\ref{fig:local_finetuning} summarizes the macro $F_1$ scores with local finetuning added at last to RealWorld, Opportunity, and PAMAP2 datasets.

\subsection{Energy profile to the baselines [R5]}
Thanks for pointing this out. We reran all experiments that involve no personalization step including FedAvg and the ablation condition of `\system{} w/o Personalization' with a new energy profile being 70\% of that with personalization. We updated the corresponding values in Figure \ref{fig:round_to_accuracy}, Figure \ref{fig:dead_devices}, Table \ref{tab:perf_summary}, and in Figure \ref{fig:rw_ablation}.


\subsection{Adding more baselines [R5]}
We added three more baseline methods: local finetuning for personalization, and \textsc{Power-of-choice}~\cite{cho2020client} and \textsc{Power-of-choice}-efficient~\cite{cho2020client} for client selection baselines. Please see \S\ref{sec:results} for details. 

\subsection{Changing the end of the experiment [R5]}
Figure~\ref{fig:round_end} shows the result of running \system{} with different sampling ratios using the PAMAP2 dataset in Figure~\ref{fig:device_count} when the end of the experiment is modified to where 230 devices become invalid. The round in which 230 devices become invalid varies from round 89 to round 864.
It shows that runs with the sampling ratio of 0.25 and 0.1 have slower convergence rates. Up to round 175 in which 230 devices run out with the sampling ratio 0.5, both models with 0.25 and 0.1 achieve significantly less macro-F1 scores. However in later rounds, they reach comparable or surpass the final accuracy of 0.5 as they continue more rounds of training while exhausting less numbers of devices.
\begin{figure}[h]
\centering
\subfloat[Round-to-accuracy]{\label{accuracy_end}\includegraphics[width=0.4\linewidth]{figures/round_to_accuracy_end.pdf}}
\subfloat[\Dead{} devices]{\label{dead_device_end}\includegraphics[width=0.4\linewidth]{figures/dead_devices_end.pdf}}
\caption{Varying the number of devices selected in each round using the PAMAP2 dataset. The experiment ran until 230 devices went invalid.}
\label{fig:round_end}
\end{figure}


\section{Questions on dataset partitioning [All]}

We first clarify the purpose of our data partitioning approach. Although there are FL dataset benchmarks such as FedScale\footnote{https://github.com/SymbioticLab/FedScale} and LEAF\footnote{https://github.com/TalwalkarLab/leaf} as pointed by R5, they neither contain any HAR datasets with inertial sensor data, nor contain any multi-device datasets. Hence, we looked for publicly available multi-device HAR datasets for our evaluation. While such datasets existed, e.g., RealWorld and Opportunity, they were collected for traditional centralized HAR training with a small number of users and each user having a large number of labeled data samples. As we explained in \S\ref{subsec:testbed}, this is not an ideal configuration for a federated setup. Firstly, it is infeasible to expect users to label large amount of accelerometer and gyroscope data on their devices (note that there is no centralized labeling in FL). Secondly, and perhaps more critically, if each client has a large number of labeled data samples, they may not even need collaborative training algorithms such as FL to train prediction models. 

As suggested by R5, we did an experiment on the RealWorld dataset to support this claim. The results in Table~\ref{tab:need_for_partition} confirm that on the original dataset (before partitioning), we can train a more accurate model with local training (macro $F_1$ = 0.88) than with FedAvg (macro $F_1$ = 0.60). Hence, the original setup, with large number of samples per user, does not benefit from FL. On the contrary, the partitioned dataset results in a low accuracy for local training (macro $F_1$ = 0.13) and we can clearly see benefits due to federated training. 

\begin{table}[h]
\caption{Macro-$F_1$ scores obtained with the RealWorld dataset. On the original dataset, with large number of samples per user, local training significantly outperforms FL. After partitioning, we can see that local training performs worse and the setup can benefit from FL.}
\begin{tabular}{@{}c|c|c@{}}
\toprule
                                                                            & \textbf{Original dataset} & \textbf{Partitioned dataset} \\ \midrule
Local Training                                                              & 0.88                      & 0.13                         \\
\begin{tabular}[c]{@{}c@{}}Federated Learning \\ (with FedAvg)\end{tabular} & 0.60                      & 0.58                         \\ \bottomrule
\end{tabular}
\label{tab:need_for_partition}
\end{table}

\parjump{}
\noindent
\uline{This finding motivated us to design a dataset partitioning scheme to make the existing multi-device HAR datasets more appropriate for federated evaluation. We will open-source the code for our partitioning scheme, and release our partitioned datasets. We also plan to contribute our datasets to extend the LEAF benchmark to HAR tasks.}


\subsection{Evaluation on FL benchmark datasets [R5]}
As noted above, although there are FL dataset benchmarks such as FedScale\footnote{https://github.com/SymbioticLab/FedScale} and LEAF\footnote{https://github.com/TalwalkarLab/leaf} as pointed by R5, they neither contain any HAR datasets with inertial sensor data, nor contain any multi-device datasets. This was one of the limitations in the benchmarks that led us to design our data partitioning scheme on existing multi-device HAR datasets. 

\subsection{Is the model learning the true classification problem? (R5)}
\label{app:classification}

R5 asked: \emph{``If the majority of the clients are inherited their classes from different sources, it can be possible that the model learned the original-client classification instead of the true classification problem. I am not familiar with HAR tasks, but it can be the case that detecting different individuals is easier than detecting different activity classes.''}

\parjump{}
\noindent
To answer this question, we investigated the features of the bottleneck layer learned by the model using TSNE plots. Our hypothesis is that if the model has inadvertently learned something about the original users, we will see clear clusters corresponding to different users in the features extracted from the data. 

\parjump{}
\noindent
Figure~\ref{user_tsne} illustrates a TSNE plot on the aggregated test set from all devices in the RealWorld dataset. Colors represent the original 15 users. We do not observe well-separated user clusters in the plot, which indicates that the model is not making its inferences based on original users. In contrast,   Figure~\ref{activity_tsne} shows a TSNE plot computed on the test data of a randomly selected participant using their personalized device model. We can clearly see clusters emerging for different activity classes, which suggests that the model has indeed learned the true activity classification problem. 

\begin{figure}[h]
\centering
\subfloat[User Separability]{\label{user_tsne}\includegraphics[width=0.49\linewidth]{figures/fail_50_forearm_1.png}} 
\subfloat[Activity Separability]{\label{activity_tsne}\includegraphics[width=0.49\linewidth]{figures/activity_tsne.png}}
\caption{TSNE Plots to illustrate user and activity separability in the bottleneck features learned by the model.}
\label{fig:tsne}
\end{figure}

\subsection{Impact of dataset generation on client selection (R5)}

R5 asks, \emph{``Data correlation is crucial for client selection strategies as well. If the clients are from the same original user, the investigated models can converge using fewer clients as the clients have preexisting knowledge of each other. Is it possible to measure how the artificial client generation makes the users' uniqueness different from a real, unprocessed dataset}?''

\parjump{}
\noindent
We measure distribution-level statistics to throw some light on this question. Specifically, we compute Sliced Wasserstein Distance (SWD)~\cite{bonneel2015sliced, rabin2011wasserstein}  between every pair of users in the original dataset as well as the partitioned RealWorld dataset. The mean SWD across users was 0.162 (original) and 0.151 (partitioned). This gives an indication that the mean distance between two users does not change significantly due to our partitioning scheme. 

\parjump{}
\noindent
Moreover, an important aspect of our device selection scheme is that it considers not just the statistical properties of a client, but also its system utilities (e.g., training time, energy consumption). Hence, even in the extreme case where two clients have exactly the same dataset, they can still have different selection probabilities due to their different system utilities. Note that our partitioning scheme only results in a partial overlap in the data across clients; therefore, we expect that each client will have a different statistical utility when training begins, and its selection probability in the subsequent rounds will be influenced by both its statistical and system utilities. 

\subsection{Advantages and Limitations of class-based data partitioning (R3)}

The main advantages of our partitioning scheme are that (a) it preserves the characteristics of the multi-device  environment (MDE), in that the synthesized users borrow different activity classes from different original users; however, within each activity class, all devices from the original users remain intact. This ensures that our partitioned dataset does not violate the definition of an MDE provided in \S\ref{sec:problem}. (b) We ensure that a new user gets data for an activity (e.g., running) from \emph{only} one of the original users. This maintains the integrity of activity classes and avoids scenarios where a synthesized user may have samples for the same activity from different original users. 


\parjump{}
\noindent
We see two potential limitations and extensions of our partitioning scheme. Firstly, as R5 highlighted, it is possible that the FL model, instead of learning the true activity classification problem, learns to classify samples based on the original users they came from. Our new empirical results in \S\ref{app:classification} highlight that this does not happen in our experiments, however one must remain careful and analyze such inadvertent information leakage in the latent space. Should such leakage happen, one can consider doing data augmentation to the activity samples before they are assigned to the synthesized users. Secondly, our partitioning scheme ensures that the synthesized users have all activity classes present in them. This can be extended to an even more challenging scenario, where newly created users have only a subset of activities present. To this end, partitioning approaches based on Dirichlet splits~\cite{dirchsplit} could be employed. We have added this explanation in the Discussion and Limitations section. 


\subsection{Does mixing users lead to worse IID? (R4)}
We measure distribution-level statistics to throw some light on this question. Specifically, we compute Sliced Wasserstein Distance (SWD)~\cite{bonneel2015sliced, rabin2011wasserstein} between every pair of users in the original dataset as well as the partitioned RealWorld dataset. The mean SWD across users was 0.162 (original) and 0.151 (partitioned). This gives an indication that the non-IID-ness does not change significantly due to our partitioning scheme. We surmise that the slight drop in SWD is caused by the data overlap between users in the partitioned dataset. 


\subsection{Inherited data from left-out users in leave-one-user-out generalizability test (R5)}
R5 questioned: \emph{``the new clients inherited data from the old clients and they are not truly unique. ... The left-out user's data is not completely new.''} 

\parjump{}
\noindent
This was not true in our leave-one-user-out (LOUO) generalizability test. We left out the randomly selected user among S1-S15 from the class-based data partitioning phase to ensure that no new users inherit data from the left-out user. Therefore, in this LOUO test, we populated synthetic users from 14 original users excluding the left-out one for training, and it was then tested on the left-out user's data. We added more explanation in the generalizability test part of \S\ref{sec:analysis_flame} to avoid confusion.



\section{Literature Review [R5]}
We elaborated explanations of client selection literature in \S\ref{sec:related_work} to a dedicated paragraph as R5 suggested. Below is the added paragraph:

\parjump{}
\noindent
\textbf{Client Selection in Federated Learning.}
Client selection strategies in FL have been proposed to optimize statistical and system utilities based on clients' data and resource information~\cite{oort, Cho2020, Nishio2019, cho2020client, dennis2021heterogeneity}.
\textsc{Power-of-choice}~\cite{cho2020client} samples highest loss clients for client selection in each round. Cho et al.~\cite{Cho2020} further present communication- and computation-efficient variants of \textsc{Power-of-choice}.
Oort~\cite{oort} also considers both statistical utility and time utility by selecting higher loss clients who can process samples within the preferred round duration.
$k$-FED~\cite{dennis2021heterogeneity} clusters data into $k$ heterogeneous clusters, which can be used as a prior to heterogeneity-aware client selection.
FedCS~\cite{Nishio2019} focuses on maximizing the number of clients to participate in a round based on the upload and update time, in scenarios where clients upload their model updates sequentially one by one. UCB-CS~\cite{Cho2020} introduces applying the discounted UCB algorithm, a multi-armed bandit algorithm, to balance the exploration-exploitation tradeoff communication-efficient client selection in FL.
We build upon the literature on client selection in FL and propose a unified client selection metric to balance model accuracy, training speed, and energy efficiency in multi-device FL.

\section{Minor revisions}
Besides the aforementioned revisions, we have completed minor revisions and corrected reference, stylistic errors, and typos as suggested by all reviewers. All changes are highlighted in blue in the paper.

